The Brown Dwarf Kinematics Project (BDKP). VI. Ultracool Dwarf Radial and Rotational Velocities from SDSS/APOGEE High-resolution Spectroscopy

We present precise measurements of radial (RV) and projected rotational ($v\sin{i}$) velocities, effective temperatures, and surface gravities of a sample of 258 M6 to L2 dwarfs with multi-epoch, high-resolution ($\lambda/\Delta\lambda$ = 22500), near-infrared (1.514-1.696 $\mu$m) spectroscopic observations reported in the Apache Point Observatory Galactic Evolution Experiment (APOGEE) Data Release 17. The spectra were modeled using a Markov Chain Monte Carlo forward-modeling method which achieved median precisions of $\sigma_\text{RV}$ = 0.4 km s$^{-1}$ and $\sigma_{v\sin{i}}$ = 1.1 km s$^{-1}$. One-half of our sample (138 sources) are previously known members of nearby young clusters and moving groups, and we identified three new kinematic members of the Argus or Carina Near moving groups, 2MASS J05402570+2448090, 2MASS J14093200+4138080, and 2MASS J21272531+5553150. Excluding these sources, we find that the majority of our sample has kinematics consistent with the Galactic thin disk, and eleven sources are associated with the intermediate thin/thick disk. The field sample has a velocity dispersion of 38.2$\pm$0.3 km s$^{-1}$, equivalent to an age of 3.30$\pm$0.19 Gyr based on empirical age-velocity dispersion relations; and a median $v\sin{i}$ of 17 km s$^{-1}$. For 172 sources with multi-epoch observations, we identified 37 as having significant radial velocity variations, and determined preliminary orbit parameters for 26 sources with four or more epochs. For 40 sources with photometric variability periods from the literature less than 5 days and $v\sin{i}$ $>$ 20 km s$^{-1}$, we find a decline in projected radii $R\sin{i}$ with age congruent with evolutionary models. Finally, we also present multi-epoch RV and vsini measurements for additional 444 candidate ultracool dwarfs.

==> table_binary_identify.tex <==
% binary identification
%\startlongtable
\begin{deluxetable*}{ccccc}
\tablecaption{Radial Velocity Variations for Multi-epoch Observations\label{table:binary_identify}}
\tabletypesize{\normalsize}
\tablehead{
\colhead{} & \colhead{} & \colhead{} & \colhead{} & \colhead{} \\ 
\colhead{APOGEE ID} & \colhead{N$_\mathrm{obs}$\tablenotemark{a}} & \colhead{Mean RV} & \colhead{$\chi^2$} & \colhead{p-value} \\ 
\colhead{} & \colhead{} & \colhead{(km s$^{-1}$)} & \colhead{} & \colhead{}
}
\startdata
2MASS J00381273$+$3850323 & $6$ & $+6.69$ & $19.45$ & $0.002$ \\ 
2MASS J03282839$+$3116273 & $10$ & $+15.25$ & $39.8$ & $<0.001$ \\ 
2MASS J03284407$+$3120528 & $18$ & $+17.41$ & $108.18$ & $<0.001$ \\ 
2MASS J03290413$+$3056127 & $17$ & $+15.53$ & $60.28$ & $<0.001$ \\ 
2MASS J03291130$+$3117175 & $15$ & $+16.57$ & $97.11$ & $<0.001$ \\ 
2MASS J03293773$+$3122024 & $19$ & $+17.02$ & $59.11$ & $<0.001$ \\ 
2MASS J03413332$+$3157417 & $17$ & $+7.45$ & $50.42$ & $<0.001$ \\ 
2MASS J03413641$+$3216200 & $4$ & $+18.56$ & $19.43$ & $<0.001$ \\ 
2MASS J03440291$+$3152277 & $12$ & $+17.53$ & $39.87$ & $<0.001$ \\ 
2MASS J03440599$+$3215321 & $7$ & $+18.85$ & $32.63$ & $<0.001$ \\ 
2MASS J04161885$+$2752155 & $4$ & $+18.43$ & $32.63$ & $<0.001$ \\ 
2MASS J04254894$+$1852479 & $3$ & $+28.28$ & $11.13$ & $0.004$ \\ 
2MASS J05402570$+$2448090 & $4$ & $+22.93$ & $28.17$ & $<0.001$ \\ 
2MASS J09373349$+$5534057 & $20$ & $+0.8$ & $109.65$ & $<0.001$ \\ 
2MASS J09453388$+$5458511 & $10$ & $-3.78$ & $22.9$ & $0.006$ \\ 
2MASS J09522188$-$1924319 & $3$ & $-17.09$ & $53.22$ & $<0.001$ \\ 
2MASS J10225090$+$0032169 & $3$ & $+34.09$ & $1172.27$ & $<0.001$ \\ 
2MASS J10541102$-$8505023 & $2$ & $-10.55$ & $45.52$ & $<0.001$ \\ 
2MASS J11203609$+$0704135 & $3$ & $-14.47$ & $11.74$ & $0.003$ \\ 
2MASS J11232934$+$0154040 & $3$ & $-0.13$ & $14.16$ & $0.001$ \\ 
2MASS J12080810$+$3520281 & $2$ & $+29.19$ & $8.46$ & $0.004$ \\ 
2MASS J12261350$+$5605445 & $5$ & $+4.13$ & $20.64$ & $<0.001$ \\ 
2MASS J12265349$+$2543556 & $8$ & $-0.25$ & $29.59$ & $<0.001$ \\ 
2MASS J12481860$-$0235360 & $14$ & $+31.27$ & $39.9$ & $<0.001$ \\ 
2MASS J13122681$+$7245338 & $10$ & $-3.47$ & $27.96$ & $0.001$ \\ 
2MASS J13202007$+$7213140 & $12$ & $-27.34$ & $35.62$ & $<0.001$ \\ 
2MASS J13232423$+$5132272 & $7$ & $-5.39$ & $17.91$ & $0.006$ \\ 
2MASS J13495109$+$3305136 & $13$ & $-9.51$ & $44.38$ & $<0.001$ \\ 
2MASS J13564148$+$4342587 & $3$ & $-19.5$ & $13.18$ & $0.001$ \\ 
2MASS J14005977$+$3226109 & $16$ & $-17.89$ & $70.77$ & $<0.001$ \\ 
2MASS J15010818$+$2250020 & $5$ & $+6.55$ & $44.72$ & $<0.001$ \\ 
2MASS J16002844$-$2209228 & $3$ & $-3.56$ & $19.69$ & $<0.001$ \\ 
2MASS J16090451$-$2224523 & $3$ & $-5.15$ & $43.57$ & $<0.001$ \\ 
2MASS J16114261$-$2525511 & $2$ & $-4.78$ & $10.0$ & $0.002$ \\ 
2MASS J16271825$+$3538347 & $4$ & $-8.56$ & $48.52$ & $<0.001$ \\ 
2MASS J22551142$+$1442456 & $5$ & $-14.27$ & $18.55$ & $0.001$ 
\enddata
\tablenotetext{a}{We regard sources with numbers of observations $<$ 4 promising candidates; see Section~\ref{sec:binaries} for more details.}
\end{deluxetable*}

==> table_binary_thejoker.tex <==
% thejoker
\begin{longrotatetable}
\startlongtable
\begin{deluxetable*}{cclcccrrcccc}
\tablecaption{Binary Orbital Parameter Estimate \label{table:binary_thejoker}}
\tabletypesize{\normalsize}
\tablehead{
\colhead{APOGEE ID} & \colhead{$N_\mathrm{obs}$} & \colhead{$P_\mathrm{Prior}$ } & \colhead{$K_\mathrm{0, Prior}$} & \colhead{$\sigma_{K_0}$} & \colhead{$\sigma_{v}$} & \colhead{$N_\mathrm{sam, in}$} & \colhead{$P_\mathrm{fit}$} & \colhead{$K_\mathrm{fit}$} & \colhead{$e_\mathrm{fit}$} & \textit{Gaia} & $\Delta$BIC \\ 
\colhead{} & \colhead{} & \colhead{(day)} & \colhead{(km s$^{-1}$)} & \colhead{(km s$^{-1}$)} & \colhead{(km s$^{-1}$)} & \colhead{} & \colhead{(day)} & \colhead{(km s$^{-1}$)} & \colhead{} & \colhead{RUWE} & \colhead{}
} 
\startdata
\hline
\multicolumn{12}{c}{$\Delta$BIC $>$ 10} \\
\hline
2M03282839$+$3116273 & 10 & 1--300 & 3.0 & 2.0 & 2.0 & 1000000 & $24.1^{+86.9}_{-21.8}$ & $1.0^{+0.3}_{-0.2}$ & $0.175^{+0.245}_{-0.132}$ & 0.995 & 32 \\ 
2M05402570$+$2448090 & 4 & 1--800 & 4.0 & 3.0 & 3.0 & 1000000 & $27.8^{+49.5}_{-24.8}$ & $2.3^{+1.2}_{-0.9}$ & $0.186^{+0.268}_{-0.143}$ & \nodata & 34 \\ 
2M08501918$+$1056436 & 23 & 1--300 & 4.0 & 3.0 & 3.0 & 5000000 & $26.0^{+17.4}_{-24.0}$ & $0.7^{+0.3}_{-0.1}$ & $0.365^{+0.43}_{-0.232}$ & 1.154 \& 1.185 & 32 \\ 
2M09442625$+$3521233 & 6 & 1--100 & 1.5 & 1.0 & 1.0 & 1000000 & $4.8^{+5.2}_{-3.4}$ & $1.2^{+0.5}_{-0.3}$ & $0.227^{+0.273}_{-0.179}$ & 0.994 & 48 \\ 
2M13430646$+$0038442 & 15 & 20--200 & 3.0 & 2.0 & 2.0 & 5000000 & $106.7^{+40.4}_{-2.0}$ & $1.1^{+0.2}_{-0.2}$ & $0.124^{+0.207}_{-0.096}$ & 1.022 & 37 \\ 
2M13482307$+$3321508 & 6 & 1--200 & 15.0 & 4.0 & 3.0 & 5000000 & $10.7^{+0.1}_{-3.4}$ & $10.8^{+3.6}_{-1.6}$ & $0.101^{+0.182}_{-0.066}$ & 1.030 & 3108 \\ 
2M13500476$+$3207596 & 15 & 1--100 & 4.0 & 3.0 & 3.0 & 5000000 & $1.7^{+0.2}_{-0.7}$ & $1.1^{+0.9}_{-0.2}$ & $0.655^{+0.093}_{-0.177}$ & 1.054 & 25 \\ 
2M14005977$+$3226109 & 16 & 1--600 & 3.0 & 3.0 & 3.0 & 5000000 & $1.4^{+321.0}_{-0.3}$ & $1.5^{+1.0}_{-0.4}$ & $0.419^{+0.258}_{-0.255}$ & 0.986 & 45 \\ 
2M15010818$+$2250020 & 5 & 5--50 & 3.0 & 3.0 & 2.0 & 1000000 & $23.3^{+1.3}_{-11.0}$ & $1.2^{+0.7}_{-0.3}$ & $0.189^{+0.284}_{-0.142}$ & 1.661 & 34 \\ 
2M16271825$+$3538347 & 4 & 60--200 & 5.0 & 4.0 & 3.0 & 5000000 & $69.7^{+17.6}_{-7.4}$ & $3.4^{+2.1}_{-1.3}$ & $0.524^{+0.175}_{-0.238}$ & 0.976 & 65 \\ 
2M16572919$+$2448509 & 4 & 100--3000 & 3.0 & 3.0 & 3.0 & 100000 & $989.0^{+1158.0}_{-800.9}$ & $0.8^{+0.6}_{-0.3}$ & $0.195^{+0.29}_{-0.15}$ & 7.898 & 20 \\ 
\hline
\multicolumn{12}{c}{$\Delta$BIC $<$ 10} \\
\hline
2M08092892$+$3235226 & 4 & 6--100 & 1.5 & 1.0 & 1.0 & 100000 & $17.7^{+11.9}_{-4.6}$ & $0.9^{+0.5}_{-0.3}$ & $0.199^{+0.255}_{-0.151}$ & 4.424 & $-1$ \\ 
2M09373349$+$5534057 & 20 & 1--100 & 4.0 & 3.0 & 2.0 & 5000000 & $5.7^{+13.5}_{-3.9}$ & $0.4^{+0.3}_{-0.2}$ & $0.271^{+0.297}_{-0.199}$ & 1.103 \& \nodata & 0 \\ 
2M09453388$+$5458511 & 10 & 1--800 & 4.0 & 3.0 & 2.0 & 5000000 & $15.1^{+119.8}_{-12.7}$ & $1.0^{+0.5}_{-0.5}$ & $0.315^{+0.298}_{-0.244}$ & 0.947 & $-1$ \\ 
2M09560888$+$0134128 & 4 & 15--800 & 1.5 & 1.0 & 1.0 & 100000 & $47.1^{+188.3}_{-25.4}$ & $1.4^{+0.7}_{-0.7}$ & $0.177^{+0.262}_{-0.14}$ & 0.929 & 6 \\ 
2M13202007$+$7213140 & 12 & 20--150 & 3.0 & 2.0 & 3.0 & 5000000 & $52.6^{+4.1}_{-16.0}$ & $0.9^{+0.6}_{-0.5}$ & $0.338^{+0.268}_{-0.213}$ & 1.332 & $-2$ \\ 
2M13232423$+$5132272 & 7 & 1--50 & 3.0 & 2.0 & 2.0 & 1000000 & $3.6^{+8.0}_{-2.0}$ & $0.7^{+0.4}_{-0.3}$ & $0.207^{+0.332}_{-0.154}$ & 1.090 \& 0.918 & 4 \\ 
2M22551142$+$1442456 & 5 & 1--50 & 3.0 & 3.0 & 2.0 & 100000 & $2.8^{+4.8}_{-1.1}$ & $1.6^{+0.9}_{-0.5}$ & $0.178^{+0.256}_{-0.135}$ & 1.091 & 5 \\
\enddata
\end{deluxetable*}
\end{longrotatetable}

==> table_kinematic_age.tex <==
% kinematic ages
%\begin{longrotatetable}
%\startlongtable
\begin{deluxetable*}{lcccccccccl}
\tablecaption{Velocity Dispersions and Group Kinematic Ages\label{table:kinematic_age}}
\tablewidth{700pt}
\tabletypesize{\scriptsize}
\tablehead{
\colhead{Sample} & \colhead{N} & \colhead{$\langle U \rangle$} & \colhead{$\langle V \rangle$} & \colhead{$\langle W \rangle$} & \colhead{$\sigma_U$} & \colhead{$\sigma_V$} & \colhead{$\sigma_W$} & \colhead{$\sigma_\mathrm{tot}$} & \colhead{Age} & \colhead{Note} \\ 
\colhead{} & \colhead{} & \colhead{(km s$^{-1}$)} & \colhead{(km s$^{-1}$)} & \colhead{(km s$^{-1}$)} & \colhead{(km s$^{-1}$)} & \colhead{(km s$^{-1}$)} &  \colhead{(km s$^{-1}$)} &  \colhead{(km s$^{-1}$)} & \colhead{(Gyr)} & \colhead{}
} 
\startdata
All & 181 & $-1.8 \pm 2.0$ & $-9.5 \pm 1.5$ & $1.9 \pm 0.9$ & $26.5 \pm 0.4$ & $19.7 \pm 0.1$ & $12.7 \pm 0.1$ & $35.4 \pm 0.4$ & $2.6 \pm 0.2$ & Unweighted \\ 
 & &  &  &  & $34.0 \pm 0.4$ & $25.6 \pm 0.2$ & $16.7 \pm 0.1$ & $45.7 \pm 0.3$ & $3.81 \pm 0.05$ & $|W|$ Weighted \\ 
% Thin Disk & 171 & $-1.9 \pm 1.9$ & $-6.9 \pm 1.1$ & $1.5 \pm 0.8$ & $25.3 \pm 0.4$ & $14.9 \pm 0.1$ & $10.4 \pm 0.1$ & $31.1 \pm 0.4$ & $1.8 \pm 0.1$ & Unweighted \\ 
% & &  &  &  & $31.9 \pm 0.4$ & $18.8 \pm 0.2$ & $13.0 \pm 0.2$ & $39.2 \pm 0.3$ & $2.7 \pm 0.1$ & $|W|$ Weighted \\ 
Not Young & 116 & $-3.1 \pm 2.9$ & $-12.4 \pm 2.2$ & $2.8 \pm 1.4$ & $31.7 \pm 0.5$ & $23.9 \pm 0.2$ & $15.6 \pm 0.1$ & $42.7 \pm 0.6$ & $4.5 \pm 0.3$ & Unweighted \\ 
 & &  &  &  & $35.5 \pm 0.4$ & $26.7 \pm 0.2$ & $17.7 \pm 0.2$ & $47.8 \pm 0.3$ & $4.19 \pm 0.05$ & $|W|$ Weighted \\ 
Thin Disk & 104 & $-3.0 \pm 3.0$ & $-8.5 \pm 1.8$ & $2.5 \pm 1.3$ & $30.5 \pm 0.6$ & $18.2 \pm 0.2$ & $12.8 \pm 0.1$ & $37.8 \pm 0.6$ & $3.2 \pm 0.2$ & Unweighted \\ 
\& Not Young & &  &  &  & $33.7 \pm 0.4$ & $19.2 \pm 0.2$ & $13.9 \pm 0.2$ & $41.2 \pm 0.4$ & $3.0 \pm 0.1$ & $|W|$ Weighted \\ 
M Dwarfs & 100 & $-3.5 \pm 3.0$ & $-8.9 \pm 1.8$ & $2.6 \pm 1.3$ & $30.0 \pm 0.6$ & $18.4 \pm 0.2$ & $12.7 \pm 0.1$ & $37.4 \pm 0.7$ & $3.1 \pm 0.2$ & Unweighted \\ 
(Thin Disk) & &  &  &  & $33.4 \pm 0.5$ & $19.5 \pm 0.2$ & $13.9 \pm 0.2$ & $41.1 \pm 0.4$ & $3.0 \pm 0.1$ & $|W|$ Weighted \\ 
L Dwarfs & 4 & $11.1 \pm 20.1$ & $2.2 \pm 3.4$ & $2.1 \pm 7.9$ & $37.4 \pm 7.4$ & $6.4 \pm 0.9$ & $14.5 \pm 3.4$ & $40.7 \pm 8.2$ & $4.3 \pm 2.4$ & Unweighted \\ 
(Thin Disk) & &  &  &  & $47.2 \pm 10.6$ & $6.9 \pm 1.0$ & $12.3 \pm 3.8$ & $49.7 \pm 9.4$ & $4.6 \pm 1.6$ & $|W|$ Weighted \\ 
Thin Disk \& & 75 & $-1.3 \pm 3.6$ & $-9.6 \pm 2.3$ & $4.1 \pm 1.5$ & $31.6 \pm 0.8$ & $19.6 \pm 0.2$ & $12.8 \pm 0.2$ & $39.3 \pm 0.8$ & $3.6 \pm 0.3$ & Unweighted \\ 
Not Young or Binary & &  &  &  & $33.6 \pm 0.6$ & $20.2 \pm 0.3$ & $14.0 \pm 0.2$ & $41.6 \pm 0.5$ & $3.1 \pm 0.1$ & $|W|$ Weighted \\
Shallow\tablenotemark{a} & 80 & $-4.6 \pm 1.9$ & $-9.7 \pm 1.2$ & $2.8 \pm 0.8$ & $30.5 \pm 0.4$ & $20.0 \pm 0.4$ & $13.6 \pm 0.2$ & $38.9 \pm 0.4$ & $3.5 \pm 0.2$ & Unweighted \\
Wide Lower\tablenotemark{a} & 16 & $-45.5 \pm 2.5$ & $-50.1 \pm 1.9$ & $-18.6 \pm 1.7$ & $34.2 \pm 2.1$ & $26.3 \pm 1.5$ & $24.3 \pm 1.1$ & $49.5 \pm 1.7$ & $6.9 \pm 0.7$ & Unweighted \\
Wide Upper\tablenotemark{a} & 16 & $44.9 \pm 3.3$ & $15.7 \pm 1.1$ & $23.9 \pm 1.6$ & $45.4 \pm 2.8$ & $15.1 \pm 0.7$ & $22.7 \pm 1.3$ & $53.0 \pm 2.5$ & $8.4 \pm 1.1$ & Unweighted \\ 
\enddata
\tablecomments{Ages for unweighted velocities and $|W|$-weighted velocities are computed with the relation and parameters from \citet{Aumer:2009aa} and \citet{Wielen:1977aa}, respectively, following the implementation in \cite{Hsu:2021aa}.}
\tablenotetext{a}{Piece-wise linear fits to unweighted velocities, broken at $\sigma = \pm 1$
%, with separate fits for sources $U = (-2.0\sigma, \, 0.0\sigma, \, 1.0\sigma, \, 2.0\sigma$), $V = (-2.0\sigma, \, -0.5\sigma, \, 1.0\sigma, \, 2.0\sigma$), and $W = (-2.0\sigma, \, -0.5\sigma, \, 0.5\sigma, \, 2.0\sigma$)
; see Section~\ref{sec:kinematic_age}.}
\end{deluxetable*}
%\end{longrotatetable}
